DC-Prophet: Predicting Catastrophic Machine Failures in DataCenters

When will a server fail catastrophically in an industrial datacenter? Is it possible to forecast these failures so preventive actions can be taken to increase the reliability of a datacenter? To answer these questions, we have studied what are probably the largest, publicly available datacenter traces, containing more than 104 million events from 12,500 machines. Among these samples, we observe and categorize three types of machine failures, all of which are catastrophic and may lead to information loss, or even worse, reliability degradation of a datacenter. We further propose a two-stage framework-DC-Prophet-based on One-Class Support Vector Machine and Random Forest. DC-Prophet extracts surprising patterns and accurately predicts the next failure of a machine. Experimental results show that DC-Prophet achieves an AUC of 0.93 in predicting the next machine failure, and a F3-score of 0.88 (out of 1). On average, DC-Prophet outperforms other classical machine learning methods by 39.45% in F3-score.

==> 060Related_Work.tex <==
%We classify the previous work into two categories as follows.
\begin{comment}

\reminder{DC: If there any previous works about anomaly detection or machine failure predictions with datacenter logs?}

\reminder{DC: If no, we should change ``Machine learning on the related datasets''}
\end{comment}

%\textbf{Data analysis on Google traces.} 
There have been many studies focusing on the machines and jobs workload and resource utilization on the Google cluster dataset \cite{chen2014failure}\cite{di2012characterization}\cite{liu2012characterizing}\cite{reiss2012heterogeneity}, while some further gave synthetic pattens which almost matched the original traces \cite{juan2014beyond}\cite{zhang2011characterizing}.  None of these works apply machine learning methods such as \ocsvm and \rf to accurately predict the next failure of a machine.
%Reiss et al. \cite{reiss2012heterogeneity} finds that many longer-running jobs has relatively stable resource utilization, which can help adaptive resource scheduling. Chen et al. \cite{chen2014failure} finds the significant differences in resource consumption between failed and finished jobs and provides Early Failure Prediction to examine how early these differences manifested in a job's lifetime, for jobs that exhibited such differences. 

%Liu et al. \cite{liu2012characterizing} analyzes a fraction from the dataset to offer first order insights and to perform a statistical analysis of node, job, and task level workload with respect to resource utilization. Wilkes et al. \cite{zhang2011characterizing} can generate synthetic workload traces that accurately reproduces resource utilization and task waiting time, by using the mean of task usage. Juan et al. \cite{juan2014beyond} discovers two key patterns of job's inter-arrivals\textemdash multiple periodicities and multi-level bundling effects. Then they propose Hierarchical Bundling Model (HIBM), which required only a handful of parameters to generate job inter-arrivals mimicking the empirical data. Konda et al. \cite{di2012characterization} compares the differences between Google data center and other Grid/HPC systems, from the perspective of machines, jobs and tasks workload.

%\textbf{Machine learning } 
Researchers have performed a number of large-scale studies on disk and machine failures using the machine learning method on the related datasets \cite{botezatu2016predicting}\cite{hamerly2001bayesian}\cite{murray2005machine}\cite{tan2010predictability}. These works have addressed only specific issues (\eg, disks) for a machine, but not for predicting the next catastrophic failure of a machine.
%Botezatu et al. \cite{botezatu2016predicting} deploys statistical techniques to automatically detect which SMART parameters correlated with disk replacement and uses them to predict the replacement of a disk with even 98\% accuracy. Hamerly et al. \cite{hamerly2001bayesian} uses two Bayesian methods to predict disk drive failures based on measurements of drive internal conditions. First, they solve the problem of anomaly detection by applying a mixture model based on Bayes cluster which is trained by using expectation-maximization. Second, they predict that a disk drive will fail if any of its snapshots are identified as anomalous by the naive Bayes classifier. 

%Murray et al. \cite{murray2005machine} compares machine learning methods to predict computer hard-drive failure using SMART attributes monitored internally by individual drives. They develop a new algorithm based on the multiple-instance learning framework and the naive Bayesian classifier (mi-NB) which is specifically designed for the low false-alarm case. Tan et al. \cite{tan2010predictability} performs an anomaly prediction approach combining feature value prediction with statistical classification methods. 



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-siggraph.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

